Compensating Removed Frequency Components: Thwarting Voice Spectrum Reduction Attacks

Automatic speech recognition (ASR) provides diverse audio-to-text services for humans to communicate with machines. However, recent research reveals ASR systems are vulnerable to various malicious audio attacks. In particular, by removing the non-essential frequency components, a new spectrum reduction attack can generate adversarial audios that can be perceived by humans but cannot be correctly interpreted by ASR systems. It raises a new challenge for content moderation solutions to detect harmful content in audio and video available on social media platforms. In this paper, we propose an acoustic compensation system named ACE to counter the spectrum reduction attacks over ASR systems. Our system design is based on two observations, namely, frequency component dependencies and perturbation sensitivity. First, since the Discrete Fourier Transform computation inevitably introduces spectral leakage and aliasing effects to the audio frequency spectrum, the frequency components with similar frequencies will have a high correlation. Thus, considering the intrinsic dependencies between neighboring frequency components, it is possible to recover more of the original audio by compensating for the removed components based on the remaining ones. Second, since the removed components in the spectrum reduction attacks can be regarded as an inverse of adversarial noise, the attack success rate will decrease when the adversarial audio is replayed in an over-the-air scenario. Hence, we can model the acoustic propagation process to add over-the-air perturbations into the attacked audio. We implement a prototype of ACE and the experiments show ACE can effectively reduce up to 87.9% of ASR inference errors caused by spectrum reduction attacks. Also, by analyzing residual errors, we summarize six general types of ASR inference errors and investigate the error causes and potential mitigation solutions.

==> summary.tex <==
\clearpage
\centerline{\bf \large Revision Summary}

\vspace{0.1in}
\noindent We thank all reviewers for the valuable comments. We have intensively revised the paper to address the concerns summarized by the shepherd and make changes promised in the rebuttal to improve the paper. The major changes are listed as follows.

\noindent{\bf Summary:}
We thoroughly revise our paper according to the comments of reviewers. To show the feasibility of two core modules, we add a new statistical experiment and provide more explanations and literature support. To clarify the experimental design and system settings, we modify the evaluation section and system overview for more clear descriptions. We revise the threat model section to add a more thorough explanation of defender's ability and possible attack variants. Besides, we revise the hypothesis of the frequency compensation module to clarify the limitations of the aliasing effect and remove the picket fence effect. Moreover, we add a description in the preliminary section to introduce the phoneme-level and word-level attacks and we revise the related work section for a better structure. We also revise the paper for the promised changes according to the comments from each individual reviewer.


%=================================================================================

\vspace{0.1in}
\noindent {\bf 1. Show the feasibility of the spectrum compensation and noise addition modules.}

\vspace{0.1in}
\noindent 
{\bf  Our Revision:}
First, in the 2nd paragraph of Section V-C, we add new experimental results of mean square errors to further clarify the feasibility of the spectrum compensation module.

\noindent{\em To better understand the spectrum compensation, we compare the mean square errors (MSE) between the benign audio and the attacked/mitigated ones. The MSE reduces from 0.030 (0.039) to 0.027 (0.036) for phoneme-level (word-level) attacks. Indeed, the compensation also adds energy to strong components and may increase MSE (this part energy has less effect on the inference); however, the compensation for the removed components can greatly recover the missing energy, hence reducing the MSE in total.}

\noindent 
Second, in the 4th paragraph of Section IV-C, we further clarify the feasibility of noise addition modules and add literature support.

\noindent{\em The voice inference of ASR systems is derived from statistical features of audio frequency spectrum. For example, the most common acoustic feature MFCC is calculated based on the energy statistics over 20 frequency bands~[24]. Thus, it is more effective to recover the spectrum statistical features, instead of the spectrum details (i.e., each individual frequency component). Because the spectrum reduction attacks change the spectrum distribution (i.e., statistical features) by removing weak components~[3], they can finally reduce the inference accuracy. However, by adding magnitude-limited noise to the attacked audio, we can fix the statistical properties of the original spectrum. That is the root reason why the noise addition module can boost the inference accuracy, even though the added noise is different from the removed energy in the spectrum details.}

%=================================================================================

\vspace{0.1in}
\noindent {\bf 2. Clarify the experimental design and settings as requested by reviewers.}

\vspace{0.1in}
\noindent {\bf Our Revision:}
First, in the fourth paragraph of Section V-A, we clarify the experimental design to show the defense models of these two ASR models are the same.

\noindent {\em Note that the adversarial audios are generated for spectrum reduction attacks with different component removal ratios and the defense models are the same for attacks against two ASR models.}

\noindent 
Second, in Section IV-A, we modify the description of the system overview to clarify the settings of \TN{}. Particularly, we list the parameters and hyperparameters used in the spectrum compensation and noise addition modules to clarify the overview of the \TN{} system before presenting the design details. Also, we modify Figure 2 to explicitly show the parameter settings used in the \TN{}.

\noindent{\em The spectrum compensation module is based on the frequency compensation strategy that aims to reconstruct the removed weak components using the remaining strong ones. In Figure~2, \TN{} estimates the original audio by the filter parameter $\alpha$, while the hyper-parameters $N$ and $L$ are spectrum and segment lengths, respectively. The noise addition module is based on the acoustic propagation strategy to introduce the over-the-air perturbations (i.e., noise with strength of $ns$) into input audio. The adaptation module focuses on detecting the attack and estimating the real spectrum removal ratio $R$, which is then used to determine the optimal parameters of $\alpha$ and $ns$ for spectrum compensation and noise addition modules.}

%=================================================================================

\vspace{0.1in}
\noindent {\bf 3. Provide a more thorough explanation of the threat model.}

\vspace{0.1in}
\noindent
{\bf Our Revision:}
In Section III, we provide a more comprehensive threat model. First, in the 2nd paragraph, we clarify defenders' capability in the training and testing phases of \TN{} system. 

\noindent{\em The \TN{} implementation includes training and testing phases. In the training phase, \TN{} can access both the original and attacked spectrums to learn the fitting parameters in each module. However, in the testing phase, \TN{} only needs to access the attacked spectrum and cannot access the original audio (i.e., ground truth).
After the processing of \TN{}, we assume that the pipeline between \TN{} and ASR is secure.}

\noindent{Second, in the 3rd paragraph of Section III, we add a description of possible attack variants.}

\noindent{\em Besides, attackers may construct different attack variants by attenuating weak component magnitude instead of removing them or removing frequencies over specific frequency bands.}

%=================================================================================

\vspace{0.1in}
\noindent {\bf 4. Explain the limitation of the aliasing effect and remove the picket fence effect.}

\vspace{0.1in}
\noindent{\bf Our Revision:}
First, in the 2nd paragraph of Section IV-B, we revise the hypothesis of DFT side effects: (1) remove the picket fence effect; (2) add brief description of spectral leakage and aliasing effects; (3) explain the limitation of aliasing effect, i.e., only applied to the undersampling devices.

\noindent{\em The spectral leakage effect introduces derived correlations to the neighboring frequency components over the computed DFT spectrum. The aliasing effect, which only occurs in devices with low sampling rates, can lead to the overlapping of frequency components.}

\noindent
Second, we modify the side effect descriptions in the introduction.

\noindent{\em First, the Discrete Fourier Transform (DFT) computation involved in the attack can introduce spectral leakage effect and sometimes aliasing effect to the audio frequency spectrum, inevitably leading to a high correlation among the frequency components with similar frequencies.}


%=================================================================================

\vspace{0.1in}
\noindent {\bf 5. Add a clear description for the phoneme/word-level attack.}

\vspace{0.1in}
\noindent{\bf Our Revision:}
In the 2nd paragraph of Section III-C, we add descriptions for phoneme/word-level attacks  before using them in the evaluation section.

\noindent{\em According to the granularity of signal segments, the attacks can be launched at either word level or phoneme level. Word-level attacks perform spectrum reduction on each word, and phoneme-level attacks take phonemes as basic units.}


%=================================================================================

\vspace{0.1in}
\noindent {\bf 6. Provide a better structure for the related work section.}

\vspace{0.1in}
\noindent{\bf Our Revision:}
In Section VIII, we restructure the related work section by using individual paragraphs with subtitle to describe each category of attacks and defenses. Also, we fix the citation issues in Section VIII.


%=================================================================================
\vspace{0.1in}
\noindent \textbf{Based on reviewers' detailed comments, we summarize our changes in the revised version as follows.}

\noindent =============================================

\noindent Review \#150A

\noindent =============================================

\vspace{0.1in}
\noindent {\bf 1. Show the feasibility of spectrum compensation and noise addition modules (requested change 1).}

\vspace{0.1in}
\noindent 
{\bf  Our Revision:}
First, in the 2nd paragraph of Section V-C, we add new experimental results of mean square errors to further clarify the feasibility of the spectrum compensation module.

\noindent{\em To better understand the spectrum compensation, we compare the mean square errors (MSE) between the benign audio and the attacked/mitigated ones. The MSE reduces from 0.030 (0.039) to 0.027 (0.036) for phoneme-level (word-level) attacks. Indeed, the compensation also adds energy to strong components and may increase MSE (this part energy has less effect on the inference); however, the compensation for the removed components can greatly recover the missing energy hence reducing the MSE in total.}

\noindent 
Second, in the 4th paragraph of Section IV-C, we further clarify the feasibility of noise addition modules and add literature support.

\noindent{\em The voice inference of ASR systems is derived from statistical features of audio frequency spectrum. For example, the most common acoustic feature MFCC is calculated based on the energy statistics over 20 frequency bands~[24]. Thus, it is more effective to recover the spectrum statistical features, instead of the spectrum details (i.e., each individual frequency component). Because the spectrum reduction attacks change the spectrum distribution (i.e., statistical features) by removing weak components~[3], they can finally reduce the inference accuracy. However, by adding magnitude-limited noise to the attacked audio, we can fix the statistical properties of the original spectrum. That is the root reason why the noise addition module can boost the inference accuracy, even though the added noise is different from the removed energy in the spectrum details.}


%=================================================================================
\vspace{0.1in}
\noindent {\bf 2. Clarify the utility of defended audios.}

\vspace{0.1in}
\noindent{\bf Our Revision:}
First, in the first paragraph of Section VII-B, we add the utility of defended audio.

\noindent{\em \TN{} aims to reduce WER/CER to the baseline level, even it is hard due to the irreversible information loss; however, reducing the flipped words/characters can still benefit content moderation systems by inferring harmful content from a more accurate context.}

\noindent
Second, in the third paragraph of Section VII-D, we point out there is no public dataset available to demonstrate the performance in real world.

\noindent{\em We are unable to evaluate the \TN{} performance with the speech understanding model due to the lack of a dataset. Such an evaluation requires a labeled dataset containing problematic content; however, existing public datasets are built for either images or text~[7], not for audio.}


%=================================================================================
\vspace{0.1in}
\noindent {\bf 3. Clarify the experimental design and settings (requested change 2).}

\vspace{0.1in}
\noindent {\bf Our Revision:}
First, in the fourth paragraph of Section V-A, we clarify the experimental design to show the defense models of these two ASR models are the same.

\noindent {\em Note that the adversarial audios are generated for spectrum reduction attacks with different component removal ratios and the defense models are the same for attacks against two ASR models.}

\noindent 
Second, in Section IV-A, we modify the description of system overview to clarify the settings of \TN{}. Particularly, we list the parameters and hyperparameters used in the spectrum compensation and noise addition modules to clarify the overview of the \TN{} system before presenting the design details. Also, we modify Figure 2 to explicitly show the parameter settings used in the \TN{}.

\noindent{\em The spectrum compensation module is based on the frequency compensation strategy that aims to reconstruct the removed weak components using the remaining strong ones. In Figure~2, \TN{} estimates the original audio by the filter parameter $\alpha$, while the hyper-parameters $N$ and $L$ are spectrum and segment lengths, respectively. The noise addition module is based on the acoustic propagation strategy to introduce the over-the-air perturbations (i.e., noise with strength of $ns$) into input audio. The adaptation module focuses on detecting the attack and estimating the real spectrum removal ratio $R$, which is then used to determine the optimal parameters of $\alpha$ and $ns$ for spectrum compensation and noise addition modules.}

%=================================================================================

\noindent =============================================

\noindent Review \#150B

\noindent =============================================

\vspace{0.1in}
\noindent {\bf 1. Explain the limitation of the aliasing effect and remove the picket fence effect (requested change 4).}

\vspace{0.1in}
\noindent{\bf Our Revision:}
First, in the 2nd paragraph of Section IV-B, we revise the hypothesis of DFT side effects: (1) remove the picket fence effect; (2) add brief description of spectral leakage and aliasing effects; (3) explain the limitation of aliasing effect, i.e., only applied to the undersampling devices.

\noindent{\em The spectral leakage effect introduces derived correlations to the neighboring frequency components over the computed DFT spectrum. The aliasing effect, which only occurs in devices with low sampling rates, can lead to the overlapping of frequency components.}

\noindent
Second, we modify the side effect descriptions in the introduction.

\noindent{\em First, the Discrete Fourier Transform (DFT) computation involved in the attack can introduce spectral leakage effect and sometimes aliasing effect to the audio frequency spectrum, inevitably leading to a high correlation among the frequency components with similar frequencies.}


%=================================================================================
\vspace{0.1in}
\noindent {\bf 2. Clarify the necessity of spectrum compensation module.}

\vspace{0.1in}
\noindent{\bf Our Revision:}
In the fifth paragraph of Section V-B, we discuss the necessity of using both modules, according to the experimental results. 

\noindent{\em Table~I also show these two modules have different mitigation effects on different data distributions, i.e., the spectrum compensation module is better over the VCTK dataset and the noise addition module is better over the TIMIT dataset. Thus, we combine two modules to achieve a better recovery effect.}



%=================================================================================
\vspace{0.1in}
\noindent{\bf 3. Explain the performance gap against word-level attacks.}

\vspace{0.1in}
\noindent{\bf Our Revision:}
In the second paragraph of Section VII-D, we add an explanation for the performance gap between phoneme-level and word-level attacks.

\noindent{\em Third, \TN{} performs well in recovering phoneme-level spectrum reduction, but yields nearly 50\% effectiveness against word-level attacks because the word-level attacks obfuscate the phoneme boundaries and cause more shifted phoneme errors. In our future work, we try to improve the ASR accuracy by recovering the phoneme boundaries of attacked audio.}



\noindent =============================================

\noindent Review \#150C

\noindent =============================================

%=================================================================================
\vspace{0.1in}
\noindent {\bf 1. Clarify we have used two ASR models.}

\vspace{0.1in}
\noindent {\bf Our Revision:}
First, in the fourth paragraph of Section V-A, we revise the first sentence to directly point out that the \TN{} performance is tested using two models.

\noindent {\em We select two open-source automatic speech recognition models DeepSpeech~[28] and CMU Sphinx~[21] in the inference stage.}

% \vspace{0.1in}
\noindent
% {\bf Our Revision 2:}
Second, in the 9th paragraph of Section I, we add the ASR usage accordingly.

\noindent{\em We prototype \TN{} and study its performance by conducting extensive experiments over two popular ASR systems (i.e., DeepSpeech~[28] and CMU Sphinx~[21]) and two public audio datasets {TIMIT}~[22] and VCTK~[51].}



%=================================================================================
\vspace{0.1in}
\noindent {\bf 2. Provide a more thorough explanation of the threat model (requested change 3).}

\vspace{0.1in}
\noindent
{\bf Our Revision:}
In Section III, we provide a more comprehensive threat model. First, in the 2nd paragraph, we clarify defenders' capability in the training and testing phases of \TN{} system. 

\noindent{\em The \TN{} implementation includes training and testing phases. In the training phase, \TN{} can access both the original and attacked spectrums to learn the fitting parameters in each module. However, in the testing phase, \TN{} only needs to access the attacked spectrum and cannot access the original audio (i.e., ground truth).
After the processing of \TN{}, we assume the pipeline between \TN{} and ASR is secure.}


%=================================================================================
\vspace{0.1in}
\noindent{\bf 3. Clarify we can access the original and attacked audio when learning the compensation model.}

\noindent{\bf Our Revision:}
In the 5th paragraph of Section IV-B, we clarify how to learn the compensation module, corresponding to the revision of the threat model in Section III.

\noindent{\em In the training phase, we obtain the scaling factors $\alpha_{i}\ (-n \leq i \leq n)$ by fitting the original and attacked spectrums. For an original spectrum $F(f)$, we can generate the attacked spectrum $A(f)$ and then utilize linear regression to obtain $\alpha$. }

\noindent{\em After obtaining the filter parameter $\alpha$, we only access the attacked audio in the testing phase. We estimate the original spectrum using $\hat{F}(f) = A(f) * \alpha$, where $*$ means convolution.}

% \sw{3. How to learn compensation model?
% In the training phase, the compensation model learns the coefficients in Equation (4) using both original and attacked audios. In the testing phase where only attacked audios are available, we estimate the spectrum reduction ratio of attacked audios and apply the corresponding coefficient.}


%=================================================================================
\vspace{0.1in}
\noindent{\bf 4. Clarify the relationship between noise parameter and component removal ratio.}

% \sw{4. Relationship between noise parameter and component removal ratio.
% Our experiments show that the best noise parameter depends on the component removal ratio, i.e., a larger component removal ratio requires a larger noise parameter. This relationship is inferred by learning from 80\% training dataset, where we have access to the original audios and the original transcripts. We will clarify this in Section V-D.}

\vspace{0.1in}
\noindent{\bf Our Revision:}
In the 2nd paragraph of Section V-D, we modify the description to clarify the relationship between component removal ratio and the best noise parameter.

\noindent{\em Our results show a larger component removal ratio requires a larger noise parameter because more energy is needed to recover the spectrum distribution. If we use a fixed noise level, the added noise can recover part of the removed components and reduce both the WER and CER of attacked audio, only if the component removal ratio is greater than a specific value. However, if the component removal ratio is less than this threshold, the added noise can negatively affect the audio and even increase the WER and CER because the added energy is greater than the removed one. Thus, the adaptation module adopts a smaller noise level for a smaller component removal ratio.}

%=================================================================================
\vspace{0.1in}
\noindent{\bf 5. Clarify we have considered the attacks via attenuating weak frequencies.}

\vspace{0.1in}
\noindent{\bf Our Revision:}
\noindent{In the 3rd paragraph of Section III, we add a description of possible attack variants, including attenuating weak frequencies.}

\noindent{\em Besides, attackers may construct different attack variants by attenuating weak component magnitude instead of removing them or removing frequencies over specific frequency bands.}

\noindent{Also, we discuss the scenarios of attenuating weak frequencies in the 2nd paragraph of Section VII-C. The detailed experimental results are shown in Appendix C and Table V.}

% \sw{5. Attenuating weak frequencies.
% In Section VII-C, we did consider the scenarios of attenuating weak frequencies instead of removing them. The performance is shown in Appendix C and Table V. ACE can handle this scenario too.}


%=================================================================================
\vspace{0.1in}
\noindent{\bf 6. Add a clear description for the phoneme/word-level attack (requested changes 5) and provide a better structure for the related work section (requested change 6).}

\vspace{0.1in}
\noindent{\bf Our Revision:}
First, in the 2nd paragraph of Section III-C, we add descriptions for phoneme/word-level attacks, before using them in the evaluation section.

\noindent{\em In addition, according to the granularity of signal segments, the attacks can be launched as word-level or phoneme-level. Word-level attacks perform spectrum reduction on each word, while phoneme-level attacks take phonemes as basic units.}

% \vspace{0.1in}
\noindent
% {\bf Our Revision 2:}
Second, in Section VIII, we provide a better structure for the related works by using individual paragraphs with sub-title to describe each category of attacks and defenses. Also, we fix the citation issues in Section VIII.

%=================================================================================

\vspace{0.1in}
\noindent{\bf *. Other minor revisions.}

% \sw{Address spelling and grammar issues throughout
% Improve the organization and presentation of the paper
% Clarify all points and make changes promised in your rebuttal}

\vspace{0.1in}
\noindent{\bf Our Revision:}
We address the typos and grammar issues in both text and figures. We also improve the content descriptions throughout the paper to make it easier to understand.


